Policy Optimization with Differentiable MPC: Convergence Analysis under Uncertainty

Model-based policy optimization is a well-established framework for designing reliable and high-performance controllers across a wide range of control applications. Recently, this approach has been extended to model predictive control policies, where explicit dynamical models are embedded within the control law. However, the performance of the resulting controllers, and the convergence of the associated optimization algorithms, critically depends on the accuracy of the models. In this paper, we demonstrate that combining gradient-based policy optimization with recursive system identification ensures convergence to an optimal controller design and showcase our finding in several control examples.

==> graphics/update_loop/update_loop_old.tex <==
\begin{tikzpicture}[thick,every node/.style={font=\footnotesize}]

\node[rectangle,very thick,rounded corners,draw=tabRed, minimum width=2.5cm, minimum height=2.25cm,fill=tabRed!15] (deploy) at (0,-0.2) {};
\node (deploy_text) at (0,0.6) {\textcolor{tabRed}{\sffamily\textbf{DEPLOY}}};

\node[rectangle,tabRed,draw,minimum height=0.5cm,minimum width=0.8cm] (f) at (0,0) {\footnotesize$f(\cdot)$};
\node[rectangle,tabRed,draw,below of=f,node distance=0.8cm,minimum height=0.5cm,minimum width=0.8cm] (mpc) {\footnotesize MPC};
\draw [-stealth,tabRed] (f.east) to [bend left=50] (mpc.east);
\draw [-stealth,tabRed] (mpc.west) to [bend left=50] (f.west);

\node[rectangle,very thick,rounded corners,draw=tabBlue, minimum width=2.5cm, minimum height=0.7cm, fill=tabBlue!15,below of =deploy, node distance = 2cm] (update) {\sffamily\textcolor{tabBlue}{\textbf{UPDATE}}};

\node[rectangle,very thick,rounded corners,draw=tabOrange, minimum width=1.7cm, minimum height=0.7cm, fill=tabOrange!15,right of = deploy, node distance = 3.5cm] (sysid) {\sffamily\textcolor{tabOrange}{\textbf{SYS-ID}}};

\draw [-{Stealth[scale=0.6]},very thick,tabRed] (deploy.east) -- node [pos=0.5, above] {\textcolor{tabRed}{$(x^k,u^k)$}} (sysid.west);
\draw [-{Stealth[scale=0.6]},very thick,tabRed] ([xshift=0.65cm]deploy.east) -- ([xshift=0.65cm,yshift=-1.85cm]deploy.east) -- ([yshift=0.15cm]update.east);
\draw [-{Stealth[scale=0.6]},very thick,tabOrange] (sysid.south) -- node [pos=0.5, right] {\textcolor{tabOrange}{$(\Theta^k,\theta^k)$}} ([yshift=-2.15cm]sysid.center) -- ([yshift=-0.15cm]update.east);
\draw [-{Stealth[scale=0.6]},very thick,tabBlue] (update.west) -- ([xshift=-0.65cm]update.west) -- node [pos=0.5,left] {\textcolor{tabBlue}{$p^k=(\tilde{p}^k,\tilde{\theta}^k)$}} ([xshift=-0.65cm]deploy.west) -- (deploy.west);

% \node [rectangle,align=center,draw,minimum height=1.2cm] (sim) at (0,0) {\scriptsize Deploy MPC on \cref{eq:system} \\ with $p=p^k$};

% \node [rectangle,draw,minimum height=1.2cm,right of=sim,node distance=2.5cm,anchor=west,align=center] (update) {\scriptsize$\begin{aligned}[c] & p^{k+1} = \mathcal{F}(p^{k},x^k,y^k,\Theta^k,\theta^k)\\
% & \Theta^{k+1},\theta^{k+1} = \mathcal{G}(\theta^k,x^k,y^k)
% \end{aligned}$};

% \draw [-latex] ([yshift=0.2cm]sim.east) -- node[pos=0.5,above] {$x^k,u^k$} ([yshift=0.2cm]update.west);

% \draw [-latex] ([yshift=0.3cm]update.east) -- ([yshift=0.3cm,xshift=0.85cm]update.east) -- ([xshift=0.85cm,yshift=-1.8cm]update.east) -- node[pos=0.75,above] {$p^k$} ([xshift=-0.45cm,yshift=-1.8cm]sim.west) -- ([xshift=-0.45cm]sim.west) -- (sim.west);

% \draw [-latex] ([yshift=-0.3cm]update.east) -- ([yshift=-0.3cm,xshift=0.45cm]update.east) -- ([xshift=0.45cm,yshift=-1.4cm]update.east) -- node[pos=0.5,above] {$\Theta^k, \theta^k$} ([xshift=-0.45cm,yshift=-1.4cm]update.west) -- ([xshift=-0.45cm,yshift=-0.2cm]update.west) -- ([yshift=-0.2cm]update.west);

\end{tikzpicture}

==> header.tex <==
% Necessary definitions for template
\def\logoname{logo}
\definecolor{subsectioncolor}{rgb}{0,0,0}
% \definecolor{subsectioncolor}{rgb}{0,0.541,0.855}
\setlength{\firstpagerule}{43pc}
\setlength{\logowidth}{0pc}
\def\journalname{IEEE TRANSACTIONS AND JOURNALS TEMPLATE}

\usepackage{textcomp}
\def\BibTeX{{\rm B\kern-.05em{\sc i\kern-.025em b}\kern-.08em
    T\kern-.1667em\lower.7ex\hbox{E}\kern-.125emX}}

% References
% \usepackage[sorting=none,style=ieee]{biblatex}
\usepackage{cite}
\usepackage{csquotes}
\usepackage[english]{babel}

% Algorithms
\RequirePackage{algorithm,algpseudocode}
\algnewcommand\algorithmicinit{\textbf{Init:}}
\algnewcommand\Init{\item[\algorithmicinit]}
\algnewcommand\algorithmicinput{\textbf{Require:}}
\algnewcommand\Input{\item[\algorithmicinput]}

% tables
\usepackage{booktabs}
\usepackage{subcaption}
\DeclareCaptionFormat{custom}
{%
    \raggedright\footnotesize #1.\, #3
}
\captionsetup{format=custom}

% Math packages
\usepackage{amssymb,amsfonts,mathrsfs}
\usepackage{amsmath}
\let\proof\relax
\let\endproof\relax
\usepackage{amsthm}
\usepackage{dsfont}
\usepackage{bm}

% SI units
\usepackage{siunitx}

% Fonts
\let\Bbbk\relax
\usepackage[cmintegrals,cmbraces,varbb]{newtxmath} % Math font
\usepackage[cal=cm,bb=ams]{mathalpha} % Improve calligraphic and bb math
\renewcommand{\ttfamily}{\fontencoding{T1}\fontfamily{lmtt}\selectfont}

% Additional math options
\usepackage{xspace}
\usepackage{derivative}

% Hyperlinks and referencing
\makeatletter
\let\NAT@parse\undefined
\makeatother
\PassOptionsToPackage{hyphens}{url}\usepackage[hidelinks]{hyperref}
\usepackage[nameinlink,sort]{cleveref}
\usepackage{bookmark}

% Figures
\usepackage[pdftex]{graphicx}

% Clever ref names
\crefname{appendix}{Appendix}{Appendices}
\AtBeginEnvironment{appendices}{\crefalias{section}{appendix}}
\crefname{assumption}{Assumption}{Assumptions}
\crefname{lemma}{Lemma}{Lemmas}
\crefname{theorem}{Theorem}{Theorems}
\crefname{problem}{Problem}{Problems}
\crefname{corollary}{Corollary}{Corollaries}
\crefname{section}{Section}{Sections}
\crefname{proposition}{Proposition}{Propositions}
\crefname{equation}{}{}
\crefmultiformat{equation}{(#2#1#3}{, #2#1#3)}{, #2#1#3}{, #2#1#3)}
\crefrangeformat{equation}{(#3#1#4-#5#2#6)}
\crefrangeformat{assumption}{Assumptions #3#1#4-#5#2#6}
\crefname{algorithm}{Algorithm}{Algorithms}
\crefname{subsection}{Section}{Sections}
\crefname{paragraph}{Paragraph}{Paragraph}
\crefname{figure}{Figure}{Figures}
\crefname{table}{Table}{Tables}
\crefname{remark}{Remark}{Remark}
\crefname{table}{Table}{Table}

% theorems
\newtheorem{theorem}{Theorem}
\newtheorem{corollary}{Corollary}
\newtheorem{proposition}{Proposition}
\newtheorem{remark}{Remark}
\newtheorem{problem}{Problem}
\theoremstyle{definition}
\newtheorem{definition}{Definition}
\newtheorem{assumption}{Assumption}
\newtheorem{lemma}{Lemma}
\newtheorem{example}{Example}

% commands for referencing problems
\newcommand{\mpc}{\hyperlink{eq:PF_MPC}{MPC$(\bar{p})$}\xspace}
\newcommand{\mpce}{\hyperlink{eq:PF_MPC}{MPC$(\bar{x}_t,p)$}\xspace}
% \newcommand{\qp}{\hyperlink{eq:DIFF_QP}{QP$(\bar{p})$}\xspace}
\newcommand{\qp}{\eqref{eq:DIFF_qp}\xspace}
% \newcommand{\dual}{\hyperlink{eq:PF_dual}{D$(\bar{p})$}\xspace}
\newcommand{\dual}{\eqref{eq:DIFF_dual}\xspace}

% Math commands
\DeclareMathOperator*{\argmin}{arg\,min}

% Counter for double columns equations
\newcounter{MYtempeqncnt}

% Project-specific definitions
\newcommand{\Rpp}{\R_{>0}}
\newcommand{\Np}{\N_{>0}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\Rx}{\mathbb{R}^{n_x}}
\newcommand{\Rp}{\mathbb{R}^{n_p}}
\newcommand{\Rn}{\mathbb{R}^{n}}
\newcommand{\Ru}{\mathbb{R}^{n_u}}
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\N}{\mathbb{N}}
\newcommand{\PPP}{\mathscr{Y}}
\newcommand{\F}{\mathcal{F}}
\newcommand{\J}{\mathcal{J}}
\renewcommand{\L}{\mathscr{L}}
\newcommand{\p}{\bar{p}}
\newcommand{\PP}{\mathscr{P}}
\newcommand{\E}{\mathbb{E}}
\newcommand{\C}{\mathbb{C}}
\newcommand{\Cb}{{\bar{\mathcal{C}}}}

% \usepackage{xcolor}
\newcommand{\eb}[1]{\textcolor{blue}{#1}}
% \newcommand{\rz}[1]{\textcolor{red}{#1}}
\newcommand{\rz}[1]{#1}

\newcommand{\tcircle}[1]{\raisebox{.5pt}{\textcircled{\raisebox{-.7pt} {#1}}}}

\newcommand{\todo}[1]{\par\noindent\textcolor{red}{\textbf{TODO}: \itshape #1}}
\newcommand{\td}{\noindent\textcolor{red}{\textbf{TODO}}}
\newcommand{\inlinetodo}[1]{\textcolor{red}{\textbf{TODO}: \itshape #1}}

% \addbibresource{bibliography.bib}

\usepackage{tikz}
\usepackage{pgfplots}
\pgfplotsset{compat=newest}
\usetikzlibrary{plotmarks}
\usetikzlibrary{shapes,arrows,decorations.markings}
\usetikzlibrary{arrows.meta}
\usepgfplotslibrary{patchplots}
\usetikzlibrary{positioning}
\usetikzlibrary{calc}
\usetikzlibrary{calligraphy}
% \usetikzlibrary{tikzmark}
\usepackage{tkz-euclide}
\pgfplotsset{tick scale binop=\times}
\def\pgfscale{0.6} % Scaling factor of matlab generated pgf plots
\usepackage{hf-tikz}
\usetikzlibrary{decorations.pathreplacing}
\usepgfplotslibrary{groupplots}
% Tikz custom blocks
\usetikzlibrary{plotmarks}
\usetikzlibrary{spy}
\usetikzlibrary{patterns}

\tikzstyle{block} = [draw, rectangle, minimum height=2.5em, minimum width=3.5em]
\tikzstyle{cblock} = [draw, rectangle, minimum height=3em, minimum width=3.5em, fill=blue!20,]
\tikzstyle{block2} = [draw, rectangle]
\tikzstyle{sum} = [draw, circle, node distance=1cm]
\tikzstyle{circ} = [draw, circle, node distance=2cm]
\tikzstyle{input} = [coordinate]
\tikzstyle{output} = [coordinate]

\tikzstyle{vecArrow} = [thick, decoration={markings,mark=at position
   1 with {\arrow[semithick]{open triangle 60}}},
   double distance=1.4pt, shorten >= 5.5pt,
   preaction = {decorate},
   postaction = {draw,line width=1.4pt, white,shorten >= 4.5pt}]
\tikzstyle{innerWhite} = [semithick, white,line width=2.6pt, shorten >= 4.5pt]


\makeatletter
\tikzset{%
  remember picture with id/.style={%
    remember picture,
    overlay,
    save picture id=#1,
  },
  save picture id/.code={%
    \edef\pgf@temp{#1}%
    \immediate\write\pgfutil@auxout{%
      \noexpand\savepointas{\pgf@temp}{\pgfpictureid}}%
  },
  if picture id/.code args={#1#2#3}{%
    \@ifundefined{save@pt@#1}{%
      \pgfkeysalso{#3}%
    }{
      \pgfkeysalso{#2}%
    }
  }
}

\def\savepointas#1#2{%
  \expandafter\gdef\csname save@pt@#1\endcsname{#2}%
}

\def\tmk@labeldef#1,#2\@nil{%
  \def\tmk@label{#1}%
  \def\tmk@def{#2}%
}

\tikzdeclarecoordinatesystem{pic}{%
  \pgfutil@in@,{#1}%
  \ifpgfutil@in@%
    \tmk@labeldef#1\@nil
  \else
    \tmk@labeldef#1,(0pt,0pt)\@nil
  \fi
  \@ifundefined{save@pt@\tmk@label}{%
    \tikz@scan@one@point\pgfutil@firstofone\tmk@def
  }{%
  \pgfsys@getposition{\csname save@pt@\tmk@label\endcsname}\save@orig@pic%
  \pgfsys@getposition{\pgfpictureid}\save@this@pic%
  \pgf@process{\pgfpointorigin\save@this@pic}%
  \pgf@xa=\pgf@x
  \pgf@ya=\pgf@y
  \pgf@process{\pgfpointorigin\save@orig@pic}%
  \advance\pgf@x by -\pgf@xa
  \advance\pgf@y by -\pgf@ya
  }%
}
\newcommand\tikzmark[2][]{%
\tikz[remember picture with id=#2] #1;}
\makeatother

\newcommand{\MarkText}[3][]{%
    \begin{tikzpicture}[overlay,remember picture]%
  \path (pic cs:#2,{(0,\paperheight)}) +(0,.7\baselineskip) coordinate (a);
  \path (pic cs:#3,{(0,-\paperheight)}) +(0,-.3\baselineskip) coordinate (b);
  \draw [ultra thick,
    if picture id={#2}{red}{line width=1cm,green,opacity=.5},
    #1]
  (a) -- ($(b)!(a)!($(b)+(1,0)$)$);
    \end{tikzpicture}%
}%

\ifmainfile
  % \usepackage{pbalance}
  \pgfplotsset{
      table/search path={graphics/data},
  }
\else
  \pgfplotsset{
      table/search path={../data},
  }
\fi

==> sources/convergence_proof.tex <==
To prove \cref{thm:main}, we first establish an explicit representation of an element of the conservative Jacobian of the penalty function $P_{\mathcal{Y}_k}$.
%
\begin{lemma}\label{lemma:jac_of_penalty}
Suppose that \cref{ass:path_diff_set} holds and that $p\notin \mathcal{Y}_k$. 
If $\gamma_\text{p}=2$, we have that
\begin{align}
2c (p-\Pi_{\mathcal{Y}_k}[p^k]) \in \J_{P_{\mathcal{Y}_k}}(p), \label{eq:convergence_proof:jac_of_penalty:ell2}
\end{align}
and if $\gamma_\text{p}=1$ we have that
\begin{align}
\frac{2c (p-\Pi_{\mathcal{Y}_k}[p^k])}{\operatorname*{dist}(p,\mathcal{Y}_k)} \in \J_{P_{\mathcal{Y}_k}}(p).\label{eq:convergence_proof:jac_of_penalty:ell1}
\end{align}
If $p\in\mathcal{Y}_k$, then $0\in \J_{P_{\mathcal{Y}_k}}(p)$.
\end{lemma}
%
\begin{proof}
We start by proving \cref{eq:convergence_proof:jac_of_penalty:ell2}.
Suppose that, leveraging \cite[Corollary 1]{bolte2021conservative}, we take $\J_{\operatorname*{dist}^2(\cdot,\mathcal{Y}_k)}=\J^c_{\operatorname*{dist}^2(\cdot,\mathcal{Y}_k)}$, where $\J_f^c$ denotes the Clarke Jacobian of $f$. Since $\mathcal{Y}_k$ is closed by \cref{ass:path_diff_set}, $\operatorname*{dist}(\cdot,\mathcal{Y}_k)$ is Lipschitz with constant $1$ by \cite[Proposition 2.4.1]{clarke1990optimization}, and therefore almost everywhere differentiable. At any point where the distance function is differentiable we have by \cite[Proposition 2.5.4]{clarke1990optimization}
\begin{align}
\nabla_p \operatorname{dist}(p,\mathcal{Y}_k) = \frac{p-\Pi_{\mathcal{Y}_k}[p^k]}{\operatorname*{dist}(p,\mathcal{Y}_k)} \label{eq:convergence_proof:jac_of_penalty:gradient_ell_1}
\end{align}
and therefore by applying the chain rule we obtain
\begin{align*}
\nabla_p \operatorname{dist}^2(p,\mathcal{Y}_k) = 2\operatorname*{dist}(p,\mathcal{Y}_k) \nabla_p \operatorname*{dist}(p,\mathcal{Y}_k) = p-\Pi_{\mathcal{Y}_k}[p^k].
\end{align*}
Let $N$ be the set of points where $\operatorname*{dist}^2(\cdot,\mathcal{Y}_k)$ is differentiable. By definition we have
\begin{align*}
& \hphantom{{}={}} \J_{\operatorname*{dist}^2(\cdot,\mathcal{Y}_k)}(p) \\
&= \operatorname*{conv}\{ \lim_{j \to \infty} \nabla_p \operatorname{dist}^2(p_j,\mathcal{Y}_k) : p_j\to p, p_j \in N\},\\
&= \operatorname*{conv}\{ \lim_{j \to \infty} p_j-\Pi_{\mathcal{Y}_k}[p_j]:p_j\to p,~p_j\in N \}\\
&= p - \operatorname*{conv}\{ \lim_{j \to \infty} \Pi_{\mathcal{Y}_k}[p_j]:p_j\to p,~p_j\in N \}
\end{align*}
By \cite[Example 7.44]{rockafellar2009variational}, we have that projectors onto closed sets are outer semicontinuous, meaning that $\{ \lim_{j \to \infty} \Pi_{\mathcal{Y}_k}[p_j]:p_j\to p,~p_j\in N \} \subset \Pi_{\mathcal{Y}_k}[p]$. We conclude that given any $\bar{p}\in \Pi_{\mathcal{Y}_k}[p]$ we have
\begin{align*}
2 (p-\bar{p}) \in \J_{\operatorname*{dist}^2(\cdot,\mathcal{Y}_k)}(p),
\end{align*}
multiplying by $c$ concludes the proof for $\gamma_\text{p}=2$. The proof for $\gamma_\text{p}=1$ follows from the same argument by utilizing \cref{eq:convergence_proof:jac_of_penalty:gradient_ell_1} without squaring the distance and from the Lipschitz continuity of $\operatorname*{dist}(p,\mathcal{Y}_k)$.

Finally, we have that $0\in \J_{P_{\mathcal{Y}_k}}(p)$ if $p\in\mathcal{Y}_k$ by recognizing that $\J^c_{\operatorname*{dist}^{\gamma_\text{p}}}(\cdot,\mathcal{Y}_k) \subset \J_{\operatorname*{dist}^{\gamma_\text{p}}}(\cdot,\mathcal{Y}_k)$ and using \cite[Theorem 2.5.6]{clarke1990optimization}.
\end{proof}
%
We now prove a technical result needed when $\gamma_\text{p}=1$.
\begin{lemma}\label{lemma:convergence:lip_continuity_jac_penalty_ell1}
Given a locally Lipschitz and definable function $f:\R^x \times \R^y \to \R^z$, and any pair of points $\bar{x}$ and $\bar{y}$, we have
\begin{align*}
    \operatorname*{dist}(\mathcal{J}_xf(x,\bar{y}),\mathcal{J}_xf(\bar{x},\bar{y})) \leq c \|x-\bar{x}\|
\end{align*}
for some $c>0$ that depends on $\bar{x}$ and $\bar{y}$ and all $x$ sufficiently close to $\bar{x}$. 
\end{lemma}
\begin{proof}
First, by definability, $f(\cdot,\bar{y})$ is piecewise twice-continuously differentiable, with finitely many (definable) pieces. If $f(\cdot,\bar{y})$ is continuously differentiable in a neighborhood of $\bar{x}$, then the result follows from the mean value theorem with $c=\|\nabla^2f(\bar{x},\bar{y})\|$.
Otherwise, $f(\cdot,\bar{y})$ is not differentiable at $\bar{x}$. In this case, by outer-semicontinuity of the conservative Jacobian $\mathcal{J}_x f(x,\bar{y})$, it holds that $\limsup_{x\to \bar{x}}\mathcal{J}_x f(x,\bar{y}) \subset \mathcal{J}_x f(\bar{x},\bar{y})$. Since $f(\cdot,\bar{y})$ is not-differentiable in finitely many points, consider a neighborhood $X$ of $\bar{x}$ such that $f(\cdot,\bar{y})$ is twice continuously differentiable everywhere in $X$ except at $\bar{x}$. Then, by the mean value theorem, for all $x\in X$ it holds that
\begin{align*}
    \| \nabla_x f(x,\bar{y}) - \lim_{x\to \bar{x}} \nabla_x f(x,\bar{y}) \| \leq \|\nabla^2 f(\xi,\bar{y})\| \|x-\bar{x}\|,
\end{align*}
where $\xi$ is a point on the line segment connecting $x$ and $\bar{x}$. The result follows by taking the supremum over $x\in X \setminus \{ x \}$.
\end{proof}
Next, we prove that $\J_{\bar{\mathcal{C}}}^k$ represents a ``sample'' of the true Jacobian $\J_\C$ of $\C$, and can thus be used to formulate a stochastic gradient descent scheme with convergence guarantees
%
\begin{lemma}\label{lemma:exchange_diff_and_exp}
Under \cref{ass:local_lip_and_definability}, the expected cost $\C(p):=\E_w[\Cb(p,w)]$ is locally Lipschitz and definable with conservative Jacobian $\J_\C(p)=\E_w[\J_\Cb(p,w)]$.
\end{lemma}
\begin{proof}
First, definability and local Lipschitz continuity are preserved by integration \cite{speissegger1999pfaffian}. Next, the function $\mathcal{C}(p,\cdot)$ is integrable for any $p$ because it is locally Lipschitz continuous. Moreover, $\J_\mathcal{C}(\cdot,w)$ is a conservative Jacobian for $\mathcal{C}(\cdot,w)$ by construction. For any given $w$, the elements of the conservative Jacobian $\J_\mathcal{C}(p,w)$ are all bounded for $p$ in bounded sets, since $\J_\mathcal{C}(\cdot,w)$ is piecewise smooth. We can therefore apply \cite[Theorem 3.10]{bolte2023subgradient} to prove the claim.
\end{proof}
%
\begin{lemma}\label{lemma:bound_gradient}
Under \cref{ass:sys_id,ass:pe,ass:local_lip_and_definability,ass:P_bounded}, there exist some $L_1>0$ such that for all $k\in\N$ and any $p\in \mathcal{P}$ and $w$, we have
\begin{align*}
\operatorname{dist}(J^k_\Cb(\theta^k),\J_{\Cb}(p^k,w^k)) \leq L_1 \operatorname*{diam}(\Theta^k),
\end{align*}
with confidence at least $1-\delta$, where $\Theta^k$ is given in \cref{eq:c_k}.
\end{lemma}
%
\begin{proof}
%
Since $\operatorname*{dist}(J^k_\Cb(\theta^k),\J_\Cb(p^k,w^k)) \leq \operatorname*{dist}(J^k_\Cb(\theta^k),J_\Cb^k) $ for any $J_\Cb^k\in\J_\Cb(p^k,w^k)$, we focus on showing that $\|J_\Cb^k(\theta^k)-J_\Cb^k\| \leq L_1 \operatorname*{diam}(\Theta^k)$ for some $L_1>0$.

Given any $k\in\N$ and $t\in\Z_{[0,T-1]}$, let $e_{u,t}^k = J_{u,t}^k(\theta^k)-J_{u,t}^k(\theta)$, $e_{x,t}^k = J_{x,t}^k(\theta^k)-J_{x,t}^k(\theta)$, and $e_{y,t}^k = J_{y,t}^k(\theta^k)-J_{y,t}^k(\theta)$. We have
\begin{align}
& \hphantom{{}={}} \|e_{x,t+1}^k\| \notag \\
& = \|J_{x,t+1}^k(\theta^k) - J_{x,t+1}^k(\theta)\| \notag \\
& \leq \|J_{f,x}^k(\theta^k) \| \| e_{x,t}^k \| + \|[J_{f,x}^k(\theta^k)-J_{f,x}^k(\theta)] J_{x,t}^k(\vartheta)\| \notag \\
& \quad~ \|J_{f,u}^k(\theta^k)\| \| e_{u,t}^k \| + \|[J_{f,u}^k(\theta^k)-J_{f,u}^k(\theta)] J_{u,t}^k(\theta)\|. \label{eq:bound0}
\end{align}
Thanks to the local Lipschitz continuity of $\mathbf{x}$ and $\mathbf{u}$ (as an immediate result from \cref{lemma:path_diff_cost}), the boundedness of $\mathcal{P}$ by \cref{ass:P_bounded}, and the fact that $w_t$ is almost surely bounded by \cref{ass:sys_id}, we can find constants $M_x$, and $M_u$ satisfying $\|J_{x,t}^k(\vartheta)\| \leq M_x$ and $\|J_{u,t}^k(\vartheta)\| \leq M_u$ for all $\vartheta\in \Theta^k$, $t\in\Z_{[0,T-1]}$, and $k\in\N$. For the same reason, there exist constants $M_{f,x}$ and $M_{f,u}$ satisfying $\|J_{f,x}(x_t^k,u_t^k,\vartheta)\| \leq M_{f,x}$ and $\|J_{f,u}(x_t^k,u_t^k,\vartheta)\| \leq M_{f,u}$ for all $\vartheta\in \Theta^k$, $t\in\Z_{[0,T-1]}$, and $k\in\N$. Let $\mathcal{X}$ be a set such that $x_t^k\in \mathcal{X}$ for all $t\in\Z_{[0,T]}$ and $k\in\N$. From \cref{eq:bound0}, we have
\begin{align}
\|e_{x,t+1}^k\| & \leq M_{f,x} \|e_{x,t}^k\| + M_{f,u} \|e_{u,t}^k\| \notag \\ & \hphantom{\leq~} + L_f (M_{u}+M_x)  \|\theta^k-\theta\|, \label{eq:bound1}
\end{align}
where $f$ is Lipschitz in $\theta$ uniformly for all $x\in \mathcal{X}$ and $u\in \mathcal{U}$ with constant $L_f$. Similarly, we have
\begin{align}
\|e_{u,t}\| \leq L_\pi [ \|e_{x,t}^k \| + \|e_{y,t}^k\| ], \label{eq:bound2}
\end{align}
where $\pi$ is Lipschitz in $(x,y)$ uniformly for $p\in \mathcal{P}$ with constant $L_\pi$, and
\begin{align}
\|e_{y,t}\| \leq L_\text{MPC} [ \| e_{x,t}^k \| + \| e_{y,t-1}^k \| ], \label{eq:bound3}
\end{align}
where $\operatorname*{MPC}$ is Lipschitz in $(x,y)$ uniformly in $p$ for all $p\in \mathcal{P}$ with constant $L_\text{MPC}$.

Since $x_0^k=\bar{x}$ and $y_{-1}^k=\bar{y}$ are fixed for all $k$, we have $e_{x,0}^k=e_{y,0}^k=0$. Suppose inductively that $e_{x,t}^k \leq L_{x,t} \|\theta^k-\theta\|$, and $e_{y,t-1}^k \leq L_{y,t-1} \|\theta^k-\theta\|$. Then from \cref{eq:bound2,eq:bound3} we have
\begin{align*}
\|e_{y,t}^k\| & \leq L_\text{MPC} ( L_{x,t} + L_{y,t-1} ) \| \theta^k-\theta \|,\\
\|e_{u,t}^k\| & \leq [ L_\pi L_{x,t} + L_\pi L_\text{MPC} (L_{x,t} + L_{y,t-1}) ] \| \theta^k-\theta \|.
\end{align*}
Letting $L_{y,t}=L_\text{MPC} ( L_{x,t} + L_{y,t-1} )$ and $L_{u,t}=L_\pi L_{x,t} + L_\pi L_\text{MPC} (L_{x,t} + L_{y,t-1})$, we obtain from \cref{eq:bound1} that
\begin{align*}
\|e_{x,t-1}^k\| \leq L_{x,t+1} \|\theta^k-\theta\|,
\end{align*}
where $L_{x,t+1}=M_{f,x} L_{x,t} + M_{f,u} L_{u,t} + L_f(M_u+M_x)$. This concludes the induction step, implying that for all $t\in\Z_{[0,T-1]}$ we have $\|e_{u,t}^k\| \leq L_u \|\theta^k-\theta\|$ and for all $t\in\Z_{[0,T]}$ we have $\|e_{x,t}^k\| \leq L_x \|\theta^k-\theta\|$.

Let $e_{x}^k=(e_{x,0}^k,\dots,e_{x,T}^k)$ and $e_u^k=(e_{u,0}^k,\dots,e_{u,T-1}^k)$. From \cref{ass:local_lip_and_definability}, we have that
\begin{align*}
& \|J_\Cb^k(\theta^k)-J_\Cb^k\| \\
\leq \, & \|J_{\mathcal{C}}^k + J_{\operatorname*{dist}(\cdot,\mathcal{X}^{T+1})}^k\| [ T L_x + (T-1) L_u ] \|\theta^k-\theta\|,
\end{align*}
where $J_\mathcal{C}^k=J_{\mathcal{C}}(x^k,u^k,p^k)$ and $J_{\operatorname*{dist}(\cdot,\mathcal{X}^{T+1})}^k \in\J_{\operatorname*{dist}(\cdot,\mathcal{X}^{T+1})}(x^k)$. Since $\mathcal{C}$ and $\operatorname*{dist}(\cdot,\mathcal{X}^{T+1})$ are locally Lipschitz, and $x^k$, $u^k$, and $p^k$ are almost surely bounded by \cref{ass:P_bounded,ass:sys_id}, there exists a constant $ L_C>0 $ such that $\|J_{\mathcal{C}}(x^k,u^k,p^k)+J_{\operatorname*{dist}(\cdot,\mathcal{X}^{T+1})}(x^k)\| \leq L_C$. Defining $L_1=L_CTL_x+L_C(T-1)L_u$ we have $\|J_\Cb^k(\theta^k)-J_\Cb^k\| \leq L_1 \|\theta^k-\theta\| \leq L_1 \operatorname*{dist}\Theta^k$ where the last statement holds with probability $1-\delta$. This completes the proof.
\end{proof}
%
\begin{lemma}\label{lemma:bound_penalty}
Under \cref{ass:path_diff_set,ass:P_bounded}, there exist some $L_2>0$ such that for all $k\in\N$ and any $p\in \mathcal{P}$
\begin{align*}
\operatorname*{dist}(\J_{P_{\mathcal{Y}}}(p),\J_{P_{\mathcal{Y}_k}}(p)) \leq L_2 \operatorname*{diam}(\Theta^k).
\end{align*}
\end{lemma}
%
\begin{proof}
We start with $\gamma_\text{p}=2$. Since by \cref{lemma:jac_of_penalty} we have $2c(p-\Pi_{\mathcal{Y}_k}[p])\in \J_{P_{\mathcal{Y}_k}}(p)$ and $2c(p-\Pi_{\mathcal{Y}}[p])\in \J_{P_{\mathcal{Y}}}(p)$, we have
\begin{align*}
\operatorname*{dist}(\J_{P_{\mathcal{Y}}}(p),\J_{P_{\mathcal{Y}_k}}(p)) &\leq \operatorname*{dist}(2c(p\!-\!\Pi_{\mathcal{Y}_k}[p]),2c(p\!-\!\Pi_{\mathcal{Y}}[p]))\\
&= 2c \operatorname*{dist}(\Pi_{\mathcal{Y}_k}[p],\Pi_{\mathcal{Y}}[p])\\
&\leq 2c \operatorname*{dist}(\mathcal{Y}_k,\mathcal{Y})\\
& \leq 2c M_2 \|\theta^k-\theta\|^{\gamma_2}.
\end{align*}
Defining $L_1 := 2c M_2$ concludes the proof for $\gamma_\text{p}=2$. The proof for $\gamma_\text{p}=1$ follows immediately from \cref{lemma:convergence:lip_continuity_jac_penalty_ell1} by recognizing that $P_{\mathcal{Y}_k}(p)=g(p,\theta_k,c_k)$, $\mathcal{P}_\mathcal{Y}(p)=g(p,\theta,0)$ and $g$ is locally Lipschitz and definable in its arguments.
\end{proof}
%
In the following, we denote $\J_{\bar{P}}^k=\J_{P_{\mathcal{Y}}}(p^k)$ and let $J_{\bar{P}}^k$ be any element of $\J_{\bar{P}}^k$.
%
\begin{proof}[Proof of \cref{thm:main}]
\textbf{Claim 1}. The update in \cref{eq:update} can be written as
\begin{align}\label{eq:proof1}
p^{k+1}= p^k+\alpha_k d^k + \alpha_k \xi^k,~~ d^k\in G_k(p^k),
\end{align}
where
\begin{align*}
G_k(p) & = -\J_{\C}(p) - \J_{\bar{P}}^k - \alpha_k^{-1}\E_w[p-\alpha_k J_\mathcal{C}(p,w) - \alpha_k J_{\bar{P}}^k \\ & \hphantom{={}} -\Pi_\mathcal{P}(p-\alpha_k J_\mathcal{C}(p,w) - \alpha_k J_{\bar{P}}^k)],\\
\alpha_k \xi^k & = \Pi_{\mathcal{P}}[p^k-\alpha_k d^k - \alpha_k J_P^k] \\ & \hphantom{={}} -\E_w[\Pi_\mathcal{P}[p^k-\alpha_k J_\mathcal{C}(p^k,w)- \alpha_k J_{\bar{P}}^k]],
\end{align*}
where $J_\mathcal{C}(p,w)\in\J_\mathcal{C}(p,w)$.

\medskip

\noindent\emph{Proof of Claim 1}. By \cref{lemma:exchange_diff_and_exp}, let $J_\C^k = \mathbb{E}_w [J_\mathcal{C}(p^k,w)] \in \J_\C(p^k)$. Then substituting
\begin{align*}
d^k=-J_\C^k-J_{\bar{P}}^k-\alpha_k^{-1}\E_w[p^k-\alpha_k J_\mathcal{C}(p^k,w)-\alpha_k J_{\bar{P}}^k]\\+\,\alpha_k^{-1}\E_w[\Pi_\mathcal{P}[p^k-\alpha_k J_\mathcal{C}(p^k,w)]-\alpha_k J_{\bar{P}}^k]
\end{align*}
in \cref{eq:proof1} yields
\begin{align*}
p^{k+1} & =  p^k - \alpha_k J_\C^k - \alpha_k J_{\bar{P}}^k - p^k + \alpha_k \E_w[J_\mathcal{C}(p^k,w)+J_{\bar{P}}^k] \\ & \hphantom{={}} + \E_w[\Pi_\mathcal{P}[p^k-\alpha_k J_\mathcal{C}(p^k,w)]-\alpha_kJ_{\bar{P}}^k] \\ & \hphantom{={}} + \Pi_{\mathcal{P}}[p^k-\alpha_k d^k- \alpha_k J_P^k] \\ & \hphantom{={}} -\E_w[\Pi_\mathcal{P}[p^k-\alpha_k J_\mathcal{C}(p^k,w)- \alpha_k J_{\bar{P}}^k]] \\
%
& = p^k - \alpha_k J_\C^k - \alpha_k J_{\bar{P}}^k - p^k + \alpha_k J_\C^k + \alpha_k J_{\bar{P}}^k \\ & \hphantom{={}} + \Pi_{\mathcal{P}}[p^k-\alpha_k d^k- \alpha_k J_P^k] \\
%
& = \Pi_{\mathcal{P}}[p^k-\alpha_k d^k - \alpha_k J_P^k].\qedhere
\end{align*}

\medskip

Next, let
\begin{align*}
\alpha_k\eta_k:=\Pi_\mathcal{P}[p_k-\alpha_k d^k-\alpha_kJ_P^k] - \Pi_\mathcal{P}[p_k-\alpha_k J_\Cb^k-\alpha_kJ_{\bar{P}}^k].
\end{align*}

\medskip

\noindent\textbf{Claim 2}. The limit $\displaystyle \lim_{n \to \infty} \sum_{k=1}^{n} \alpha_k \eta_k$ exists and it is finite.

\medskip

\noindent\emph{Proof of Claim 2}. We use \cite[Proposition 4.32]{bonnans2013perturbation} by showing that all assumptions are verified. Let $k\in\N$ be fixed. Let $\Phi=\mathcal{P}$, $f_k(p)=\|p-p^k+\alpha_k J_\Cb^k+\alpha_kJ_{\bar{P}}^k\|^2$ and $g_k(p)=\|p-p^k+\alpha_k d^k+\alpha J_P^k\|^2$. Observe that
\begin{enumerate}
    \item Since $\nabla^2 f_k(p)=2I$, for any $p,p'$
    \begin{align*}
    f(p') \geq f_k(p) + \nabla f_k(p) ^{\top} (p-p') + \|p-p'\|^2,
    \end{align*}
    If $p\in\argmin_{x\in\Phi} f_k(x)$, then $\nabla f_k(p) ^{\top} d \geq 0$ for all locally feasible directions $d \neq 0$, i.e., those $d \neq 0$ such that there exists some $\epsilon>0$ for which $x+td\in \Phi$ for all $t\in (0,\epsilon]$ \cite[Theorem 4.9]{bagirov2014introduction}. Therefore, if $p'$ is sufficiently close to $p$, then $\nabla f_k(p)^{\top}(p-p') \geq 0$ and therefore $f$ satisfies the quadratic growth property
    \begin{align*}
    f_k(p') \geq f_k(p) + \|p-p'\|^2.
    \end{align*}
    \item We have
    \begin{align*}
    & \| \nabla f_k(p) - \nabla g_k(p) \| \\
    =~ & 2\| p\!-\!p^k\!+\!\alpha_k J_\Cb^k\!+\!\alpha_k J_{\bar{P}}^k \!-\! p + p^k \!-\! \alpha_k d^k\!-\!\alpha_k J_P^k\| \\
    \leq~ & 2 \alpha_k [ \| J_\Cb^k-d^k \| + \| J_{\bar{P}}^k - J_P^k \| ] \\
    \leq~ & 2 \alpha_k (L_1 + L_2) \operatorname*{diam}\Theta^k + 2 \alpha_k^2 =: \kappa,
    \end{align*}
    where the last step follows from \cref{lemma:bound_gradient,lemma:bound_penalty}. This means that $f_k-g_k$ is $\kappa$-Lipschitz.
\end{enumerate}
Let $S_0$ be the set of minimizers of the problem $\min_{p\in \Phi} ~f_k(p)$, and let $S_1$ be the set of minimizers of the problem $\min_{p\in \Phi}~ g_k(p)$. Observe that $\alpha_k \| \eta_k \| \leq \operatorname*{dist} (S_0,S_1) $. From \cite[Proposition 4.32]{bonnans2013perturbation} we have that for all $k$ large enough, say for all $k \geq \bar{k}$,
\begin{align*}
\operatorname*{dist}(S_0,S_1) \leq \kappa = 2 \alpha_k^2 + 2 \alpha_k(L_1+L_2) \operatorname*{diam}\Theta^k.
\end{align*}
We conclude that for all $k \geq \bar{k}$, $\alpha_k \eta_k \leq 2 \alpha_k^2 + 2 \alpha_k(L_1+L_2) \operatorname*{diam}\Theta^k$. By \cref{ass:stepsizes}, $\sum_{k=\bar{k}}^{\infty} 2 \alpha_k^2 < \infty$. By \cref{thm:sys_id}, there exists some $C>0$ for which $\operatorname*{diam}\Theta^k \leq C \sqrt{\log k / k} $. Therefore, $\sum_{k=\bar{k}}^{\infty} 2 \alpha_k(L_1+L_2) \operatorname*{diam}\Theta^k \leq 2C(L_1+L_2) \sum_{k=\bar{k}}^{\infty} \alpha_k \sqrt{\log k / k} < \infty$. We conclude that $\lim_{n \to \infty} \sum_{k=1}^{n} \alpha_k \eta_k < \infty$.

\medskip

\noindent\textbf{Claim 3}. The limit $\displaystyle \lim_{n \to \infty} \sum_{k=1}^{n} \alpha_k \xi^k$ exists.

\medskip

\noindent\emph{Proof of Claim 3}. We have $\alpha_k \xi^k = \alpha_k \eta_k + \alpha_k \varphi_k$, where $\alpha_k \varphi_k := \Pi_\mathcal{P}[p^k-\alpha_k J_\mathcal{C}^k] - \E_w[\Pi_\mathcal{P}[p^k-\alpha_k J_\mathcal{C}(p^k,w)]]$. The limit $\lim_{n \to \infty} \sum_{k=1}^{n} \alpha_k \varphi_k$ exists by \cref{lemma:exchange_diff_and_exp} and \cite[Lemma A.5]{davis2020stochastic}, and $\alpha_k \eta_k$ is summable by Claim 2.

\medskip

Combining Claims 1 to 3 with \cite[Lemmas A.6 and A.7]{davis2020stochastic}, we conclude that Assumption A in \cite{davis2020stochastic} holds. Since also Assumption B in \cite{davis2020stochastic} holds, by the definability of the objective function and by \cref{lemma:Yk_is_definable}, the Theorem follows from \cite[Theorem 3.2]{davis2020stochastic}.
\end{proof}
